An Analysis of Multilingual FActScore

FActScore has gained popularity as a metric to estimate the factuality of long-form texts generated by Large Language Models (LLMs) in English. However, there has not been any work in studying the behavior of FActScore in other languages. This paper studies the limitations of each component in the four-component pipeline of FActScore in the multilingual setting. We introduce a new dataset for FActScore on texts generated by strong multilingual LLMs. Our evaluation shows that LLMs exhibit distinct behaviors in both fact extraction and fact scoring tasks. No LLM produces consistent and reliable FActScore across languages with varying levels of resources. We also find that the knowledge source plays an important role in the quality of the estimated FActScore. Using Wikipedia as the knowledge source may hinder the true FActScore of long-form text due to its limited coverage in medium- and low-resource languages. We also incorporate three mitigations to our knowledge source that ultimately improve FActScore estimation across all languages.

==> tables/context_unfaithful_gemini.tex <==
\begin{table}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llcrrrc}
    \toprule
        \bf Lang & \bf Subject model & \bf \# of samples & \bf Context unfaithful & \bf Annotation error & \bf Bad retrieval & \bf Task/annotation design  & \bf Information in table & \bf Debatable & \bf Being filtered & \bf Assistant generation & \bf Inconsistant Wikipedia\\
        \midrule
        \mtr{2}{Spanish} & GemP & 30 & 13 & 1 & 10 & 1 & 2 & 3 & 0 & 0 & 0\\
                         & GPT4 & 30 & 8 & 2 & 8 & 1 & 6 & 4 & 0 & 1 & 0\\
                         & Both & 60 & 21 & 3 & 18 & 2 & 8 & 7 & 0 & 1 & 0\\
        \midrule
        \mtr{2}{Arabic}  & GemP & 30 & 12 & 2 & 4 & 3 & 6 & 1 & 1 & 0 & 1\\
                         & GPT4 & 30 & 14 & 2 & 3 & 0 & 6 & 3 & 0 & 2 & 0\\
                         & Both & 60 & 26 & 4 & 7 & 3 & 12 & 4 & 1 & 2 & 0\\
        \midrule
        \mtr{2}{Bengali} & GemP & 30 & 12 & 3 & 4 & 0 & 7 & 3 & 1 & 0 & 0\\
                         & GPT4 & 30 & 15 & 1 & 4 & 0 & 5 & 4 & 1 & 0 & 0\\
                         & Both & 30 & 27 & 4 & 8 & 0 & 12 & 7 & 2 & 0 & 0\\
        \bottomrule
    \end{tabular}
}
\caption{Disparity reasons between native annotators and Gemini-Pro by 60 disagreement samples}
\label{tab:context_unfaithful_gemini}
\end{table}

==> tables/disagreement_example_by_gemini_bn.tex <==
\begin{table*}[!h]
\small
    \centering
    \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}p{0.65\linewidth}}
    \toprule
        \bf Category & \bf Fact & \bf Comment\\
        \midrule
        \bf Context unfaithful - Factually correct & \langbn{তিনি হলিউড ওয়াক অফ ফেমে তারকা পেয়েছেন।.}
        
        {\bf Translated:} {\it ``He received a star on the Hollywood Walk of Fame.''} & Native label: F, Model label: T, Ground truth: T.
        
        {\bf Comment:} No related information within the provided Wikipedia page. But there is supporting evidence from https://walkoffame.com/tom-hanks/.\\
        \midrule
        \bf Context unfaithful - Hallucination & “দ্য ও.সি. ২০০৬-২০০৭ সালে প্রচারিত হয়েছিল।” 
        
        {\bf Translated:} {\it ``The OC aired in 2006-2007.''} & Native label: F, Model label: T, Ground truth: F.
        
         {\bf Comment:} The fact is false based on information from the series' Wikipedia page.
         
         {\bf Evidence:} The O.C. is an American teen drama television series created by Josh Schwartz that originally aired on the Fox network in the United States from August 5, 2003, to February 22, 2007, with a total of four seasons consisting of 92 episodes.\\
        \midrule
        \bf Context unfaithful - Reading Deficiency & "বিদ্যাধর সূর্যপ্রসাদ নাইপল." 
        
        {\bf Translated:} {\it ``Naipaul moved to England as a teenager.''} & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} The evaluator misses the related information (that supports the fact) within retrieved passages.
        
        {\bf Evidence:} "তিনি ১৯৫০ অক্সফোর্ড বিশ্ববিদ্যালয়ে ভর্তি হন এবং ইংরেজি সাহিত্য বিষয়ে অধ্যয়ন করেন।" ({\bf en:} "He entered Oxford University in 1950 and studied English literature.")\\
        \midrule
        \bf Retrieval error &  "নেইমার ব্রাজিলের সান্তোস এফসি একাডেমিতে তার ক্যারিয়ারের শুরু করেন।" 
        
        {\bf Translated:} {\it ``Neymar started his career at Santos FC academy in Brazil.''} & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} The retriever fails to retrieve the needed information passage for evaluation.
        
        {\bf Evidence:} "নেইমার খুব কম বয়সেই ফুটবল খেলা আরম্ভ করেন। খুব অল্প সময়েই তিনি সান্তোস ফুটবল ক্লাব কর্তৃপক্ষের নজরে আসেন।" 
        
        ({\bf en:} "Neymar started playing football at a very young age. In a very short time, he came to the attention of Santos Football Club authorities.")\\
        \midrule
        \bf Tabular data & "\"গুড বয়, ব্যাড বয়\" ছবিটি ২০০৭ সালে মুক্তি পায়।" {\bf Translated:} {\it ``The film \"Good Boy, Bad Boy\" was released in 2007.''} & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} Related information is embedded in the table which is not processed by Wikipedia's HTML conversion to text, thus not being contained as passages to retrieve.
        
        {\bf Evidence:} Information locates at চলচ্চিত্রের তালিকা (List of movies) section, the third row.\\
        \midrule
        \bf Subjective opinion & তিনি সান্টোসের সাথে 10টি ব্রাজিলীয় লিগ শিরোপা জিতেছেন।" 
        
        {\bf Translated:} {\it ``He won 10 Brazilian league titles with Santos.''} & Native label: T, Model label: F, Ground truth: T/F.
        
        {\bf Comment:} There are two versions Brazilian league from two organizations. Therefore, the calculation of the total number of titles won by the team could be different based on which version or if the sum of both is considered.\\
        % \midrule
        % \bf Annotation error & "ব্লুমফিল্ড একটি বিশেষ ধারণা পোষণ করতেন।" {\bf Translated:} {\it ``Bloomfield held a particular opinion.''} & Native label: F, Model label: T, Ground truth: T.
        
        % {\bf Comment:} Leonard Bloomfield did have an opinion and personal perspective on the object of research in linguistics (should only be linguistics not mind, as he stated)
        
        % {\bf Evidence:} "টি বর্জন করে ভাষাবিজ্ঞানকে আচরণবাদের মূল কেন্দ্র হিসেবে প্রতিষ্ঠা করার চেষ্টা করেন। তিনি বক্তার মানসিক সংগঠনের অস্তিত্ত্ব সম্পূর্ণ উপেক্ষা করেন এবং বলেন যে মানুষের মুখের উচ্চারিত ভাষার বিভিন্ন ধ্বনি, শব্দ ও বাক্যের কাঠামো উদ্ঘাটনই ভাষাবিজ্ঞানের গবেষণার একমাত্র বিষয়।" ({\bf en:} "Tried to establish linguistics as the core of behaviorism by rejecting T. He completely ignores the existence of the speaker's mental organization and says that the study of linguistics is the sole purpose of linguistics to uncover the various sounds, words and sentence structures of spoken language.")\\
        \bottomrule
    \end{tabular}
\caption{Examples from each disagreement categories between natives and Gemini in Spanish.}
\label{tab:example_disgreement_gemini_bn}
\end{table*}


==> tables/disagreement_example_by_gpt4_bn.tex <==
\begin{table*}[!h]
\small
    \centering
    \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}p{0.65\linewidth}}
    \toprule
        \bf Category & \bf Fact & \bf Comment\\
        \midrule
        \bf Context unfaithful - Factually correct & “তার অধ্যয়নের স্থান ছিল টেনেসি বিশ্ববিদ্যালয়।” (en: “His place of study was University of Tennessee.”) & Native label: F, Model label: T, Ground truth: T.
        
        {\bf Comment:} No related information within the provided Wikipedia page. But there is supporting evidence from en.wikipedia.
        
        {\bf Evidence:} McCarthy was born in Providence, Rhode Island, although he was raised primarily in Tennessee. In 1951, he enrolled in the University of Tennessee, but dropped out to join the U.S. Air Force.\\
        \midrule
        \bf Context unfaithful - Hallucination & “টাভারে তার টেস্ট ক্যারিয়ারে 1,735 রান করেছেন।” (en: “Avere scored 1,735 runs in his Test career.”) & Native label: F, Model label: T, Ground truth: F.
        
         {\bf Comment:} The fact is false. scored 1,755 runs in his Test career.\\
        \midrule
        \bf Context unfaithful - Reading Deficiency & "ম্যাকার্থির লেখালেখির প্রাথমিক কাল ছিল।" (en: “McCarthy had an early period of writing.”) & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} The evaluator misses the related information (that supports the fact) within retrieved passages.
        
        {\bf Evidence:} "নব্বইয়ের দশকে লেখা "বর্ডার উপন্যাসত্রয়ী" তার সেরা সৃষ্টি।" ({\bf en:} ""Border novel" written in the nineties is his best work.")\\
        \midrule
        \bf Retrieval error & "তাঁর কারাদণ্ডের মেয়াদ ছিল পাঁচ বছর।" (en: “The term of his imprisonment was five years.”) & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} The retriever fails to retrieve needed information passage for evaluation.
        
        {\bf Evidence:} "দক্ষিণ আফ্রিকার বর্ণবাদী শ্বেতাঙ্গ সরকার ১৯৫৬ খ্রিষ্টাব্দের ৫ ডিসেম্বর তারিখে ম্যান্ডেলাসহ ১৫০ জন বর্ণবাদবিরোধী কর্মীকে দেশদ্রোহিতার অপরাধে গ্রেপ্তার করে। এই মামলাটি সুদীর্ঘ ৫ বছর ধরে (১৯৫৬-১৯৬১) চলে, কিন্তু মামলার শেষে সব আসামি নির্দোষ প্রমাণিত হন।" ({\bf en:} "South Africa's apartheid white government arrested 150 anti-apartheid activists, including Mandela, on charges of treason on December 5, 1956. The case lasted for 5 long years (1956-1961), but at the end of the trial all the accused were found innocent.")\\
        \midrule
        \bf Tabular data & "টুয়েন্টি২০ ম্যাচে 25 ম্যাচ খেলা হয়েছে।" (en: “25 matches played in Twenty20.”) & Native label: T, Model label: F, Ground truth: T.
        
        {\bf Comment:} Related information is embedded in the table which is not processed by Wikipedia's HTML conversion to text, thus not being contained as passages to retrieve.
        
        {\bf Evidence:} Information locates on খেলোয়াড়ী জীবনের পরিসংখ্যান (Player life statistics) section of the side infobox.\\
        % \midrule
        % \bf Annotation error & "ব্লুমফিল্ডের পদ্ধতি ভাষাবিজ্ঞানে একটি বড় পরিবর্তন আনে।" (en: “Bloomfield's method marks a major change in linguistics.”) & Native label: T, Model label: F, Ground truth: F.
        
        % {\bf Comment:} The annotator missed details.
        
        % {\bf Evidence:} "রূপমূলতত্ত্বে ব্লুমফিল্ড বিভিন্ন ধরনের ধ্বনিতাত্ত্বিক পরিবর্তনের উপর সচেতনভাবে মনোযোগ দেন, যার ফলশ্রুতিতে আধুনিক রূপধ্বনিমূলতত্ত্ব প্রতিষ্ঠা হয়। বাক্যতত্ত্বে ব্লুমফিল্ড উপাদান কাঠামো (constituent structure)-এর তত্ত্বের ভিত্তি স্থাপন করেন।" ({\bf en:} "In etymology Bloomfield consciously focused on various types of phonological change, resulting in the establishment of modern phonological etymology. Bloomfield laid the foundations of the theory of constituent structure in syntax.")\\
        \bottomrule
    \end{tabular}

\caption{Examples from each disagreement categories between natives and GPT-4 in Bengali.}
\label{tab:example_disgreement_gpt4_bn}
\end{table*}





==> tables/disagreement_reason_gemini.tex <==
% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llclllp{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.13\linewidth}}
%     \toprule
%         \bf Lang & \bf Subject model & \bf \#samples & \multicolumn{3}{c}{\bf Unfaithful} & \bf Annotation & \bf Retrieval & \bf Design & \bf Table & \bf Debatable & \bf Filtered & \bf Assistant & \bf Inconsistent\\
%         \cmidrule(r){4-6}
%         & & & \bf Correct & \bf Hallucinate & \bf Reading\\
%         \midrule
%         \multirow{3}{*}{Spanish} & GemP & 30 (11, 19) & 8 (8, 0) & 0 (0, 0) & 5 (0, 5) & 1 (0, 1) & 10 (0, 10) & 1 (1, 0) & 2 (0, 2) & 3 (2, 1) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0)\\
%                          & GPT-4 & 30 (9, 21) & 4 (4, 0) & 0 (0, 0) & 4 (0, 4) & 2 (1, 1) & 8 (0, 8) & 1 (1, 0) & 6 (1, 5) & 4 (1, 3) & 0 (0, 0) & 1 (1, 0) & 0 (0, 0)\\
%                          & Both & 60 (20, 40) & 12 (12, 0) & 0 (0, 0) & 9 (0, 9) & 3 (1, 2) & 18 (0, 18) & 2 (2, 0) & 8 (1, 7) & 7 (3, 4) & 0 (0, 0) & 1 (1, 0) & 0 (0, 0)\\
%         \midrule
%         \multirow{3}{*}{Arabic}  & GemP & 30 (13, 17) & 4 (4, 0) & 1 (1, 0) & 7 (3, 4) & 2 (1, 1) & 4 (0, 4) & 3 (2, 1) & 6 (1, 5) & 1 (0, 1) & 1 (0, 1) & 0 (0, 0) & 1 (1, 0)\\
%                          & GPT-4 & 30 (13, 17) & 7 (7, 0) & 1 (1, 0) & 6 (0, 6) & 2 (1, 1) & 3 (1, 2) & 0 (0, 0) & 6 (0, 6) & 3 (1, 2) & 0 (0, 0) & 2 (2, 0) & 0 (0, 0)\\
%                          & Both & 60 (26, 34) & 11 (11, 0) & 2 (2, 0) & 13 (3, 10) & 4 (2, 2) & 7 (1, 6) & 3 (2, 1) & 12 (1, 11) & 4 (1, 3) & 1 (0, 1) & 2 (2, 0) & 1 (1, 0)\\
%         \midrule
%         \multirow{3}{*}{Bengali} & GemP & 30 (21, 9) & 5 (5, 0) & 2 (2, 0) & 5 (0, 5) & 3 (1, 2) & 4 (0, 4) & 0 (0, 0) & 7 (0, 7) & 3 (1, 2) & 1 (0, 1) & 0 (0, 0) & 0 (0, 0)\\
%                          & GPT-4 & 30 (8, 22) & 7 (4, 3) & 2 (2, 0)  & 6 (0, 6) & 1 (0, 1) & 4 (0, 4) & 0 (0, 0) & 5 (0, 5) & 4 (2, 2) & 1 (0, 1) & 0 (0, 0) & 0 (0, 0)\\
%                          & Both & 60 (26, 34) & 12 (9, 3) & 4 (4, 0) & 11 (0, 11) & 4 (1, 3) & 8 (0, 8) & 0 (0, 0) & 12 (0, 12) & 7 (3, 4) & 2 (0, 2) & 0 (0, 0) & 0 (0, 0)\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and Gemini-Pro from 60 disagreement samples. Reasons include Context unfaithful (Unfaithful) (consists of Factually correct (Correct), Hallucinate (Hallucinate), Reading deficiency (Reading)), Annotation error (Annotation), Bad Retrieval (Retrieval), Task/annotation design (Design), Information in table (Table), Debatable (Debatable), Being filtered (Filtered), Assistant generation (Assistant), Inconsistent Wikipedia (Inconsistent). Each cell is represented by [\#samples (\#False Positives, \#False Negatives)]. True/false positive/negative with native annotations as labels, modelling evaluations as predictions}
% \label{tab:qualitative_analysis_gemini}
% \end{table*}



% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llclllp{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.5\linewidth}p{0.12\linewidth}p{0.12\linewidth}}
%     \toprule
%         \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Unfaithful} & \bf Annotation & \bf Retrieval & \bf In table & \bf Debatable & \bf Others\\
%         \cmidrule(r){4-6}
%         & & & \bf Correct & \bf Hallucinate & \bf Reading\\
%         \midrule
%         \multirow{3}{*}{Spanish} & GemP & 30 (11, 19) & 8 (8, 0) & 0 (0, 0) & 5 (0, 5) & 1 (0, 1) & 10 (0, 10) & 2 (0, 2) & 3 (2, 1) & 1\\
%                          & GPT-4 & 30 (9, 21) & 4 (4, 0) & 0 (0, 0) & 4 (0, 4) & 2 (1, 1) & 8 (0, 8) & 6 (1, 5) & 4 (1, 3) & 2\\
%                          & Both & 60 (20, 40) & 12 (12, 0) & 0 (0, 0) & 9 (0, 9) & 3 (1, 2) & 18 (0, 18) & 8 (1, 7) & 7 (3, 4) & 3\\
%         \midrule
%         \multirow{3}{*}{Arabic}  & GemP & 30 (13, 17) & 4 (4, 0) & 1 (1, 0) & 7 (3, 4) & 2 (1, 1) & 4 (0, 4) & 6 (1, 5) & 1 (0, 1) & 5\\
%                          & GPT-4 & 30 (13, 17) & 7 (7, 0) & 1 (1, 0) & 6 (0, 6) & 2 (1, 1) & 3 (1, 2) & 6 (0, 6) & 3 (1, 2) & 2\\
%                          & Both & 60 (26, 34) & 11 (11, 0) & 2 (2, 0) & 13 (3, 10) & 4 (2, 2) & 7 (1, 6) & 12 (1, 11) & 4 (1, 3) & 7\\
%         \midrule
%         \multirow{3}{*}{Bengali} & GemP & 30 (21, 9) & 5 (5, 0) & 2 (2, 0) & 5 (0, 5) & 3 (1, 2) & 4 (0, 4) & 7 (0, 7) & 3 (1, 2) & 1\\
%                          & GPT-4 & 30 (8, 22) & 7 (4, 3) & 2 (2, 0)  & 6 (0, 6) & 1 (0, 1) & 4 (0, 4) & 5 (0, 5) & 4 (2, 2) & 1\\
%                          & Both & 60 (26, 34) & 12 (9, 3) & 4 (4, 0) & 11 (0, 11) & 4 (1, 3) & 8 (0, 8) & 12 (0, 12) & 7 (3, 4) &2\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and Gemini-Pro from 60 disagreement samples. Reasons include Context unfaithful (Unfaithful) (consists of Factually correct (Correct), Hallucinate (Hallucinate), Reading deficiency (Reading)), Annotation error (Annotation), Bad Retrieval (Retrieval), Information in table (In table), Debatable (Debatable) and Others (Others). Each cell is represented by [\#samples (\#False Positives, \#False Negatives)]. True/false positive/negative with native annotations as labels, modelling evaluations as predictions}
% \label{tab:qualitative_analysis_gemini}
% \end{table*}

\begin{table*}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llclllp{0.12\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
    \toprule
        \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
        \cmidrule(r){4-6}
        & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
        \midrule
        \multirow{3}{*}{Spanish} & GemP & 30 & 8 & 0 & 5 & 1 & 10 & 2 & 3 & 1\\
                         & GPT-4 & 30 & 4 & 0 & 4 & 2 & 8 & 6 & 4 & 2\\
                         & Both & 60 & 12 & 0 & 9 & 3 & 18 & 8 & 7 & 3\\
        \midrule
        \multirow{3}{*}{Arabic}  & GemP & 30 & 4 & 1 & 7 & 2 & 4 & 6 & 1 & 5\\
                         & GPT-4 & 30 & 7 & 1 & 6 & 2 & 3 & 6 & 3 & 2\\
                         & Both & 60 & 11 & 2 & 13 & 4 & 7 & 12 & 4 & 7\\
        \midrule
        \multirow{3}{*}{Bengali} & GemP & 30 & 5 & 2 & 5 & 3 & 4 & 7 & 3 & 1\\
                         & GPT-4 & 30 & 7 & 2  & 6 & 1 & 4 & 5 & 4 & 1\\
                         & Both & 60 & 12 & 4 & 11 & 4 & 8 & 12 & 7 & 2\\
        \bottomrule
    \end{tabular}
}
\caption{Disparity reasons between native annotators and GemP from 60 disagreement samples.}
\label{tab:qualitative_analysis_gemini}
\end{table*}


 % Reasons include Context unfaithful (Unfaithful) (consists of Factually correct (Correct), Hallucinate (Hallucinate), Reading deficiency (Reading)), Annotation error (Annotation), Bad Retrieval (Retrieval), Information in table (In table), Debatable (Debatable) and Others (Others). Each cell is represented by [\#samples (\#False Positives, \#False Negatives)]. True/false positive/negative with native annotations as labels, modelling evaluations as predictions

==> tables/disagreement_reason_gpt4.tex <==
% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llcrrrrrrrrrrr}
%     \toprule
%         \bf Lang & \bf Subject model & \bf \#samples & \multicolumn{3}{c}{\bf Context unfaithful} & \bf Annotation error & \bf Bad retrieval & \bf Task/annotation design & \bf Information in table & \bf Debatable & \bf Being filtered & \bf Assistant generation & \bf Inconsistent Wikipedia\\
%         \cmidrule(r){4-6}
%         & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
%         \midrule
%         \multirow{3}{*}{Spanish} & GemP & 30 (23, 7) & 12 (12, 0) & 4 (4, 0) & 2 (1, 1) & 1 (1, 0) & 1 (0, 1) & 2 (2, 0) & 2 (0, 2) & 4 (3, 1) & 2 (0, 2) & 0 (0, 0) & 0 (0, 0)\\
%                          & GPT4 & 30 (26, 4) & 17 (17, 0) & 6 (6, 0) & 0 (0, 0) & 1 (0, 1) & 1 (0, 1) & 0 (0, 0) & 0 (0, 0) & 2 (2, 0) & 2 (2, 0) & 1 (1, 0)  & 0 (0, 0)\\
%                          & Both & 60 (49, 11) & 29 (29, 0) & 10 (10, 0) & 2 (1, 1) & 2 (0, 2) & 2 (1, 1) & 2 (2, 0) & 2 (0, 2) & 6 (5, 1) & 4 (2, 2) & 1 (1, 0) & 0 (0, 0)\\
%         \midrule
%         \multirow{3}{*}{Arabic}  & GemP & 30 (22, 8) & 14 (14, 0) & 5 (5, 0) & 3 (0, 3) & 0 (0, 0) & 4 (0, 4) & 3 (3, 0) & 1 (0, 1) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0)\\
%                          & GPT4 & 30 (27, 3) & 17 (17, 0) & 4 (4, 0) & 2 (0, 2) & 1 (1, 0) & 0 (0, 0) & 1 (1, 0) & 1 (0, 1) & 3 (3, 0) & 0 (0, 0) & 1 (1, 0) & 0 (0, 0)\\
%                          & Both & 60 (49, 11) & 31 (31, 0) & 9 (9, 0) & 5 (0, 5) & 1 (1, 0) & 4 (0, 4) & 4 (4, 0) & 2 (0, 2) & 3 (3, 0) & 0 (0, 0) & 1 (1, 0) & 0 (0, 0)\\
%         \midrule
%         \multirow{3}{*}{Bengali} & GemP & 30 (21, 9) & 18 (18, 0) & 1 (1, 0) & 0 (0, 0) & 3 (1, 2) & 3 (0, 3) & 3 (1, 2) & 2 (0, 2) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0)\\
%                          & GPT4 & 30 (25, 5) & 22 (22, 0) & 3 (3, 0) & 2 (0, 2) & 1 (0, 1) & 0 (0, 0) & 0 (0, 0) & 2 (0, 2) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0)\\
%                          & Both & 60 (46, 14) & 40 (40, 0) & 4 (4, 0) & 2 (0, 2) & 4 (1, 3) & 3 (0, 3) & 3 (1, 2) & 4 (0, 4) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0) & 0 (0, 0)\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and GPT-4 from 60 disagreement samples. Each cell is represented by [\#samples (\#False Positives, \#False Negatives)]. True/false positive/negative with native annotations as labels, modelling evaluations as predictions}
% \label{tab:qualitative_analysis_gpt4}
% \end{table*}


% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llclllp{0.12\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
%     \toprule
%         \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
%         \cmidrule(r){4-6}
%         & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
%         \midrule
%         \multirow{3}{*}{Spanish} & GemP & 30 (23, 7) & 12 (12, 0) & 4 (4, 0) & 2 (1, 1) & 1 (1, 0) & 1 (0, 1) & 2 (0, 2) & 4 (3, 1)\\
%                          & GPT4 & 30 (26, 4) & 17 (17, 0) & 6 (6, 0) & 0 (0, 0) & 1 (0, 1) & 1 (0, 1) & 0 (0, 0) & 2 (2, 0)\\
%                          & Both & 60 (49, 11) & 29 (29, 0) & 10 (10, 0) & 2 (1, 1) & 2 (0, 2) & 2 (1, 1) & 2 (0, 2) & 6 (5, 1)\\
%         \midrule
%         \multirow{3}{*}{Arabic}  & GemP & 30 (22, 8) & 14 (14, 0) & 5 (5, 0) & 3 (0, 3) & 0 (0, 0) & 4 (0, 4) & 1 (0, 1) & 0 (0, 0)\\
%                          & GPT4 & 30 (27, 3) & 17 (17, 0) & 4 (4, 0) & 2 (0, 2) & 1 (1, 0) & 0 (0, 0) & 1 (0, 1) & 3 (3, 0)\\
%                          & Both & 60 (49, 11) & 31 (31, 0) & 9 (9, 0) & 5 (0, 5) & 1 (1, 0) & 4 (0, 4) & 2 (0, 2) & 3 (3, 0)\\
%         \midrule
%         \multirow{3}{*}{Bengali} & GemP & 30 (21, 9) & 18 (18, 0) & 1 (1, 0) & 0 (0, 0) & 3 (1, 2) & 3 (0, 3) & 2 (0, 2) & 0 (0, 0)\\
%                          & GPT4 & 30 (25, 5) & 22 (22, 0) & 3 (3, 0) & 2 (0, 2) & 1 (0, 1) & 0 (0, 0) & 2 (0, 2) & 0 (0, 0)\\
%                          & Both & 60 (46, 14) & 40 (40, 0) & 4 (4, 0) & 2 (0, 2) & 4 (1, 3) & 3 (0, 3) & 4 (0, 4) & 0 (0, 0)\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and GPT-4 from 60 disagreement samples.}
% \label{tab:qualitative_analysis_gpt4}
% \end{table*}


\begin{table*}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llclllp{0.12\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
    \toprule
        \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
        \cmidrule(r){4-6}
        & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
        \midrule
        \multirow{3}{*}{Spanish} & GemP & 30 & 12 & 4 & 2 & 1 & 1 & 2 & 4 & 4\\
                         & GPT4 & 30 & 17 & 6 & 0 & 1 & 1 & 0 & 2 & 3\\
                         & Both & 60 & 29 & 10 & 2 & 2 & 2 & 2 & 6 & 7\\
        \midrule
        \multirow{3}{*}{Arabic}  & GemP & 30 & 14 & 5 & 3 & 0 & 4 & 1 & 0 & 3\\
                         & GPT4 & 30 & 17 & 4 & 2 & 1 & 0 & 1 & 3 & 2\\
                         & Both & 60 & 31 & 9 & 5 & 1 & 4 & 2 & 3 & 5\\
        \midrule
        \multirow{3}{*}{Bengali} & GemP & 30 & 18 & 1 & 0 & 3 & 3 & 2 & 0 & 3\\
                         & GPT4 & 30 & 22 & 3 & 2 & 1 & 0 & 2 & 0 & 0\\
                         & Both & 60 & 40 & 4 & 2 & 4 & 3 & 4 & 0 & 3\\
        \bottomrule
    \end{tabular}
}
\caption{Disparity reasons between native annotators and GPT4 from 60 disagreement samples.}
\label{tab:qualitative_analysis_gpt4}
\end{table*}

==> tables/disagreement_reason_merged.tex <==
% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{lllclllp{0.12\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
%     \toprule
%         \bf Evaluator & \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
%         \cmidrule(r){5-7}
%         & & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
%         \midrule
%         \multirow{9}{*}{GemP} & \multirow{3}{*}{Spanish} & GemP & 30 & 8 & 0 & 5 & 1 & 10 & 2 & 3 & 1\\
%                          & & GPT-4 & 30 & 4 & 0 & 4 & 2 & 8 & 6 & 4 & 2\\
%                          & & Both & 60 & 12 & 0 & 9 & 3 & 18 & 8 & 7 & 3\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{Arabic}  & GemP & 30 & 4 & 1 & 7 & 2 & 4 & 6 & 1 & 5\\
%                          & & GPT-4 & 30 & 7 & 1 & 6 & 2 & 3 & 6 & 3 & 2\\
%                          & & Both & 60 & 11 & 2 & 13 & 4 & 7 & 12 & 4 & 7\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{Bengali} & GemP & 30 & 5 & 2 & 5 & 3 & 4 & 7 & 3 & 1\\
%                          & & GPT-4 & 30 & 7 & 2  & 6 & 1 & 4 & 5 & 4 & 1\\
%                          & & Both & 60 & 12 & 4 & 11 & 4 & 8 & 12 & 7 & 2\\
%         \midrule
%         \multirow{9}{*}{GPT4} & \multirow{3}{*}{Spanish} & GemP & 30 & 12 & 4 & 2 & 1 & 1 & 2 & 4 & 4\\
%                          & & GPT4 & 30 & 17 & 6 & 0 & 1 & 1 & 0 & 2 & 3\\
%                          & & Both & 60 & 29 & 10 & 2 & 2 & 2 & 2 & 6 & 7\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{Arabic}  & GemP & 30 & 14 & 5 & 3 & 0 & 4 & 1 & 0 & 3\\
%                          & & GPT4 & 30 & 17 & 4 & 2 & 1 & 0 & 1 & 3 & 2\\
%                          & & Both & 60 & 31 & 9 & 5 & 1 & 4 & 2 & 3 & 5\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{Bengali} & GemP & 30 & 18 & 1 & 0 & 3 & 3 & 2 & 0 & 3\\
%                          & & GPT4 & 30 & 22 & 3 & 2 & 1 & 0 & 2 & 0 & 0\\
%                          & & Both & 60 & 40 & 4 & 2 & 4 & 3 & 4 & 0 & 3\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and modeling evaluators (GemP/GPT4) from 60 disagreement samples (facts).}
% \label{tab:qualitative_analysis_merged}
% \end{table*}


% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llp{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
%     \toprule
%         \bf Evaluator & \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
%         \cmidrule(r){5-7}
%         & & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
%         \midrule
%         \multirow{9}{*}{GemP} & \multirow{3}{*}{es} & GemP & \large 30 & \large 8 & \large 0 & \large 5 & \large 1 & \large 10 & \large 2 & \large 3 & \large 1\\
%                          & & GPT4 & \large 30 & \large 4 & \large 0 & \large 4 & \large 2 & \large 8 & \large 6 & \large 4 & \large 2\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{ar}  & GemP & \large 30 & \large 4 & \large 1 & \large 7 & \large 2 & \large 4 & \large 6 & \large 1 & \large 5\\
%                          & & GPT4 & \large 30 & \large 7 & \large 1 & \large 6 & \large 2 & \large 3 & \large 6 & \large 3 & \large 2\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{bn} & GemP & \large 30 & \large 5 & \large 2 & \large 5 & \large 3 & \large 4 & \large 7 & \large 3 & \large 1\\
%                          & & GPT4 & \large 30 & \large 7 & \large 2 & \large 6 & \large 1 & \large 4 & \large 5 & \large 4 & \large 1\\
%         \midrule
%         \multirow{9}{*}{GPT4} & \multirow{3}{*}{es} & GemP & \large 30 & \large 12 & \large 4 & \large 2 & \large 1 & \large 1 & \large 2 & \large 4 & \large 4 \\
%                          & & GPT4 & \large 30 & \large 17 & \large 6 & \large 0 & \large 1 & \large 1 & \large 0 & \large 2 & \large 3\\
%         \cmidrule{2-12}
%         & \multirow{2}{*}{ar}  & GemP & \large 30 & \large 14 & \large 5 & \large 3 & \large 0 & \large 4 & \large 1 & \large 0 & \large 3\\
%                          & & GPT4 & \large 30 & \large 17 & \large 4 & \large 2 & \large 1 & \large 0 & \large 1 & \large 3 & \large 2\\
%         \cmidrule{2-12}
%         & \multirow{2}{*}{bn} & GemP & \large 30 & \large 18 & \large 1 & \large 0 & \large 3 & \large 3 & \large 2 & \large 0 & \large 3\\
%                          & & GPT4 & \large 30 & \large 22 & \large 3 & \large 2 & \large 1 & \large 0 & \large 2 & \large 0 & \large 0\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and modeling evaluators (GemP/GPT4) from 60 disagreement samples (facts).}
% \label{tab:qualitative_analysis_merged}
% \end{table*}



% \begin{table}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llp{0.12\linewidth}p{0.12\linewidth}p{0.12\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.10\linewidth}p{0.13\linewidth}p{0.11\linewidth}p{0.10\linewidth}}
%     \toprule
%         \bf Evaluator & \bf Lang & \bf Subject model & \bf \#samples (facts) & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Annotation Error & \bf Bad retrieval & \bf Information in table & \bf Debatable & \bf Others\\
%         \cmidrule(r){5-7}
%         & & & & \bf Factually correct & \bf Hallucinate & \bf Reading deficiency\\
%         \midrule
%         \multirow{9}{*}{GemP} & \multirow{3}{*}{es} & GemP & 30 & 8 & 0 & 5 & 1 & 10 & 2 & 3 & 1\\
%                          & & GPT4 & 30 & 4 & 0 & 4 & 2 & 8 & 6 & 4 & 2\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{ar}  & GemP & 30 & 4 & 1 & 7 & 2 & 4 & 6 & 1 & 5\\
%                          & & GPT4 & 30 & 7 & 1 & 6 & 2 & 3 & 6 & 3 & 2\\
%         \cmidrule{2-12}
%         & \multirow{3}{*}{bn} & GemP & 30 & 5 & 2 & 5 & 3 & 4 & 7 & 3 & 1\\
%                          & & GPT4 & 30 & 7 & 2  & 6 & 1 & 4 & 5 & 4 & 1\\
%         \midrule
%         \multirow{9}{*}{GPT4} & \multirow{3}{*}{es} & GemP & 30 & 12 & 4 & 2 & 1 & 1 & 2 & 4 & 4\\
%                          & & GPT4 & 30 & 17 & 6 & 0 & 1 & 1 & 0 & 2 & 3\\
%         \cmidrule{2-12}
%         & \multirow{2}{*}{ar}  & GemP & 30 & 14 & 5 & 3 & 0 & 4 & 1 & 0 & 3\\
%                          & & GPT4 & 30 & 17 & 4 & 2 & 1 & 0 & 1 & 3 & 2\\
%         \cmidrule{2-12}
%         & \multirow{2}{*}{bn} & GemP & 30 & 18 & 1 & 0 & 3 & 3 & 2 & 0 & 3\\
%                          & & GPT4 & 30 & 22 & 3 & 2 & 1 & 0 & 2 & 0 & 0\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and modeling evaluators (GemP/GPT4) from 60 disagreement samples (facts).}
% \label{tab:qualitative_analysis_merged}
% \end{table}




\begin{table}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccccc}
    \toprule
    & \bf Subject & \multicolumn{3}{c}{\bf Context Unfaithful} & \bf Ret. & \bf Tab. & \bf Deb. & \bf Misc.\\
    \cmidrule(r){3-5}
    & & \bf FC & \bf Hal. & \bf RD\\
    \midrule
    \multirow{3}{*}{es} 
        & GemP &   8 &  0 &  5 &   10 &  2 &  3 &  1\\
        & GPT4 &   4 &  0 &  4 &   8 &  6 &  4 &  2\\
    \cmidrule{2-9}
    \multirow{3}{*}{ar}  
        & GemP &   4 &  1 &  7 &    4 &  6 &  1 &  5\\
        & GPT4 &   7 &  1 &  6 &  3 &  6 &  3 &  2\\
    \cmidrule{2-9}
    \multirow{3}{*}{bn} 
        & GemP &   5 &  2 &  5  &  4 &  7 &  3 &  1\\
        & GPT4 &   7 &  2 &  6 &    4 &  5 &  4 &  1\\
    \midrule
    \multirow{3}{*}{es} 
        & GemP &   12 &  4 &  2  &  1 &  2 &  4 &  4 \\
        & GPT4 &   17 &  6 &  0 &   1 &  0 &  2 &  3\\
    \cmidrule{2-9}
    \multirow{2}{*}{ar}  
        & GemP &   14 &  5 &  3 &    4 &  1 &  0 &  3\\
        & GPT4 &   17 &  4 &  2 &    0 &  1 &  3 &  2\\
    \cmidrule{2-9}
    \multirow{2}{*}{bn} 
        & GemP &   18 &  1 &  0 &    3 &  2 &  0 &  3\\
        & GPT4 &   22 &  3 &  2 &    0 &  2 &  0 &  0\\
    \bottomrule
\end{tabular}
}
\caption{Disparity reasons between native annotators and modeling evaluators (GemP/GPT4) from 60 disagreement samples (facts).}
\label{tab:qualitative_analysis_merged}
\end{table}

==> tables/fact_extractor_comparison.tex <==
% \begin{table}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llcrrrrrrr}
%     \toprule
%         \bf & \bf Fact & \bf \#Sent & \bf Merge & \bf Split & \bf Grounded & \bf Dup. & \bf Insufficient & \bf Ling. & \bf Avg.\\
%         & \bf Extractor & & & & & & & \bf Error &  \\
%         \midrule
%         \mtr{3}{es} & GPT-3.5 & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%                      & Gemma & 192 & 0 & 35 & 0 & 0 & 14 & 0 & 5.74\\
%                      & GPT-4 & 192 & 1 & 2 & 0 & 3 & 9 & 0 & 5.92\\
%         \midrule
%         \mtr{3}{ar}  & GPT-3.5 & 180 & 1 & 22 & 10 & 2 & 13 & 3 & 5.72\\
%                      & Gemma & 180 & 0 & 20 & 10 & 0 & 14 & 2 & 5.74\\
%                      & GPT-4 & 180 & 3 & 0 & 5 & 0 & 8 & 0 & 5.9\\
%         \midrule
%         \mtr{3}{bn} & GPT-3.5 & 175 & 3 & 36 & 19 & 12 & 24 & 8 & 5.41\\
%                      & Gemma & 175 & 2 & 22 & 5 & 2 & 7 & 1 & 5.74\\
%                      & GPT-4 & 175 & 2 & 9 & 3 & 2 & 8 & 0 & 5.86\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Assessment of language models as extractors considering six aspects. For each error, the extractor's score is subtracted by 1 point. \hl{@Kim: Do not use this score, just report the average number of errors}}
% \label{tab:fact_extractor}
% \end{table}



\begin{table}[!ht]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llcrrrrrrc}
    \toprule
        \bf & \bf Extractor & \bf \#Sent & \bf M & \bf S & \bf G  & \bf D & \bf I & \bf L & \bf Avg.\\
        \midrule
        \mtr{3}{es} & GPT-3.5 & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 0.25\\
                     & FT Gemma & 192 & 0 & 35 & 0 & 0 & 14 & 0 & 0.26\\
                     & GPT-4 & 192 & 1 & 2 & 0 & 3 & 9 & 0 & 0.08\\
        \midrule
        \mtr{3}{ar}  & GPT-3.5 & 180 & 1 & 22 & 10 & 2 & 13 & 3 & 0.28\\
                     & FT Gemma & 180 & 0 & 20 & 10 & 0 & 14 & 2 & 0.26\\
                     & GPT-4 & 180 & 3 & 0 & 5 & 0 & 8 & 0 & 0.09\\
        \midrule
        \mtr{3}{bn} & GPT-3.5 & 175 & 3 & 36 & 19 & 12 & 24 & 8 & 0.58\\
                     & FT Gemma & 175 & 2 & 22 & 5 & 2 & 7 & 1 & 0.22\\
                     & GPT-4 & 175 & 2 & 9 & 3 & 2 & 8 & 0 & 0.14\\
        \bottomrule
    \end{tabular}
}
\caption{Assessment of language models as extractors considering six aspects (Need merge (M), Need Split, Not Grounded (G), Duplicated (D), Insufficient (I), and Linguistic Error (L)), and the average number of errors per sentence on texts generated by subject models: GPT4 and GemP .}
\label{tab:fact_extractor}
\end{table}

==> tables/knowledge_source_capacity.tex <==
\begin{table}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llcrrrc}
    \toprule
        \bf Lang & \bf Average \# of facts & \bf Average \# of passages\\
        \midrule
        \mtr{2}{Spanish} & 391.6 & 15.5\\
        \midrule
        \mtr{2}{Arabic}  & 317.5 & 13.0\\
        \midrule
        \mtr{2}{Bengali} & 277.3 & 12.8\\
        \bottomrule
    \end{tabular}
}
\caption{Statistics of knowledge source utilized by FActScore pipeline in three languages including average number of facts and average number of passages (256 tokens each) per each Wikipedia page}
\label{tab:biography_generation}
\end{table}

==> tables/new_method_comparison.tex <==
% \begin{table}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llcrrrr}
%     \toprule
%         \bf Lang & \bf Method & \multicolumn{2}{c}{\bf FActScore} & \multicolumn{3}{c}{\bf Agreement with golden labelling}\\
%         \cmidrule(r){3-4} & \cmidrule(r){5-7}
%         & & \bf On Gemini's generated facts & \bf On GPT-4's generated facts & \bf On Gemini's generated facts & \bf On GPT-4's generated facts & \bf On both's generated facts\\
%         \midrule
%         \mtr{7}{Spanish} & Gemini with 1 Wikipage (5 passage) & 58.81 & 68.39 & 70.32 & 69.83 & 70.07\\
%                          & Gemini with 1 Wikipage (8 passage) & 63.29 & 72.84 & 74.34 & 73.99 & 74.16\\
%                          & Gemini with 1 Wikipage (20 passage) & 67 & 77.3 & 77.28 & 78.45 & 77.89\\
%                          & Gemini with Google Search (SAFE) & 81.45 & 90.3 & 83.23 & 89.87 & 86.67\\
%                          & Gemini with knowledge generated by GPT-4 & 78.83 & 93.46 & 84.62 & 91.88 & 88.38\\
%                          & Natives with Wikipedia & 75.27 & 88.36 & 91.89 & 90.05 & 91.4\\
%                          & Natives with the Internet & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         % \midrule
%         % \mtr{6}{Arabic}  & Gemini with 1 Wikipage (8 passage) & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Gemini with 1 Wikipage (20 passage) & 192 & 1 & 2 & 0 & 3 & 9 & 0 & 5.92\\
%         %                  & Gemini with Google Search (SAFE) & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Gemini with knowledge generated by GPT-4 & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Natives with Wikipedia & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Natives with the Internet & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         % \midrule
%         % \mtr{6}{Bengali} & Gemini with 1 Wikipage (8 passage) & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Gemini with 1 Wikipage (20 passage) & 192 & 1 & 2 & 0 & 3 & 9 & 0 & 5.92\\
%         %                  & Gemini with Google Search (SAFE) & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Gemini with knowledge generated by GPT-4 & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Natives with Wikipedia & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         %                  & Natives with the Internet & 192 & 1 & 24 & 0 & 9 & 14 & 0 & 5.75\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Disparity reasons between native annotators and Gemini-Pro from 60 disagreement samples. Each cell is represented by [\#samples (\#False Positives, \#False Negatives)]. True/false positive/negative with native annotations as labels, modelling evaluations as predictions}
% \label{tab:qualitative_analysis_gemini}
% \end{table*}


% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llcrrrr}
%     \toprule
%         \bf Lang & \bf Method & \multicolumn{2}{c}{\bf FActScore} & \multicolumn{3}{c}{\bf Agreement with golden labelling (\#False positives, \#False negatives)}\\
%         \cmidrule(r){3-4} \cmidrule(r){5-7}
%         & & \bf On Gemini's generated facts & \bf On GPT-4's generated facts & \bf On Gemini's generated facts & \bf On GPT-4's generated facts & \bf On both's generated facts\\
%         \midrule
%         \mtr{7}{Spanish} & Gemini with 1 Wikipage (5 passage) & 58.81 & 68.39 & 70.32 (36, 348) & 69.83 (9, 411) & 70.07 (45, 759)\\
%                          & Gemini with 1 Wikipage (8 passage) & 63.29 & 72.84 & 74.34 (39, 293) & 73.99 (11, 351) & 74.16 (50, 644)\\
%                          & Gemini with 1 Wikipage (20 passage) & 67 & 77.3 & 77.28 (44, 250) & 78.45 (11, 289) & 77.89 (50, 644)\\
%                          & Gemini with Google Search (SAFE) & 81.45 & 90.3 & 83.23 (99, 118) & 89.87 (22, 119) & 86.67 (121, 237)\\
%                          & Gemini with knowledge generated by GPT-4 & 78.83 & 93.46 & 84.62 (73, 126) & 91.88 (30, 83) & 88.38 (103, 209)\\
%                          & Natives with Wikipedia & 75.27 & 88.36 & 91.89 (3, 62) & 90.05 (1, 79) & 91.4 (4, 141) \\
%                          & Natives with the Internet & 82.92 & 97.27 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Arabic} & Gemini with 1 Wikipage (8 passage) & 56.4 & 73.71 & 77.91 (52, 212) & 78.33 (15, 187) & 78.09 (67, 399)\\
%                          & Gemini with 1 Wikipage (20 passage) & 60.59 & 76.72 & 79.92 (65, 175) & 81.12 (16, 160) & 80.44 (81, 335)\\
%                          & Gemini with Google Search (SAFE) & 72.3 & 87.66 & 80.25 (138, 101) & 86.27 (56, 82) & 82.89 (194, 183)\\
%                          & Gemini with knowledge generated by GPT-4 & 64.44 & 82.4 & 83.6 (66, 130) & 84.66 (26, 117) & 84.06 (92, 247)\\
%                          & Natives with Wikipedia & 60.92 & 81.87 & 90.79 (3, 69) & 89.7 (2, 43) & 90.31 (5, 112)\\
%                          & Natives with the Internet & 69.21 & 90.45 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Bengali} & Gemini with 1 Wikipage (8 passage) & 43.78 & 52.97 & 60.61 (4, 265) & 55.12 (1, 271) & 58.03 (5, 536)\\
%                          & Gemini with 1 Wikipage (20 passage) & 52.56 & 63.53 & 69.11 (5, 206) & 65.68 (1, 207) & 67.49 (6, 413)\\
%                          & Gemini with Google Search (SAFE) & 75.55 & 87.95 & 86.82 (23, 67) & 87.79 (8, 66) & 87.28 (31, 133)\\
%                          & Gemini with knowledge generated by GPT-4 & 59.44 & 69.97 & 74.82 (9, 163) & 71.12 (4, 171) & 73.08 (13, 334)\\
%                          & Natives with Wikipedia & 57.83 & 61.22 & 74.08 (6, 154) & 62.71 (3, 163) & 68.74 (9, 317)\\
%                          & Natives with the Internet & 81.99 & 97.52 & 100 & 100 & 100\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{FActScore and agreement with golden labelling of introduced methods namely increasing \# of passages, using GPT-4 to generate knowledge source and using Gemini as a Google search agent and evaluator, comparison with the baseline and native annotations. Comparison is conducted on Gemini's generated facts (Gemini), GPT-4's generated facts (GPT-4) and a combine of both (Both).}
% \label{tab:compare_proposed_method}
% \end{table*}

% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llcrrrr}
%     \toprule
%         \bf Lang & \bf Method & \multicolumn{2}{c}{\bf FActScore} & \multicolumn{3}{c}{\bf Agreement with golden labelling}\\
%         \cmidrule(r){3-4} \cmidrule(r){5-7}
%         & & \bf Gemini & \bf GPT-4 & \bf Gemini & \bf GPT-4 & \bf Both\\
%         \midrule
%         \mtr{7}{Spanish} & Gemini with 1 Wikipage (5 passage) & 58.81 & 68.39 & 70.32 (36, 348) & 69.83 (9, 411) & 70.07 (45, 759)\\
%                          & Gemini with 1 Wikipage (8 passage) & 63.29 & 72.84 & 74.34 (39, 293) & 73.99 (11, 351) & 74.16 (50, 644)\\
%                          & Gemini with 1 Wikipage (20 passage) & 67 & 77.3 & 77.28 (44, 250) & 78.45 (11, 289) & 77.89 (50, 644)\\
%                          & Gemini with Google Search (SAFE) & 81.45 & 90.3 & 83.23 (99, 118) & 89.87 (22, 119) & 86.67 (121, 237)\\
%                          & Gemini with knowledge generated by GPT-4 & 78.83 & 93.46 & 84.62 (73, 126) & 91.88 (30, 83) & 88.38 (103, 209)\\
%                          & Natives with Wikipedia & 75.27 & 88.36 & 91.89 (3, 62) & 90.05 (1, 79) & 91.4 (4, 141) \\
%                          & Natives with the Internet & 82.92 & 97.27 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Arabic} & Gemini with 1 Wikipage (8 passage) & 56.4 & 73.71 & 77.91 (52, 212) & 78.33 (15, 187) & 78.09 (67, 399)\\
%                          & Gemini with 1 Wikipage (20 passage) & 60.59 & 76.72 & 79.92 (65, 175) & 81.12 (16, 160) & 80.44 (81, 335)\\
%                          & Gemini with Google Search (SAFE) & 72.3 & 87.66 & 80.25 (138, 101) & 86.27 (56, 82) & 82.89 (194, 183)\\
%                          & Gemini with knowledge generated by GPT-4 & 64.44 & 82.4 & 83.6 (66, 130) & 84.66 (26, 117) & 84.06 (92, 247)\\
%                          & Natives with Wikipedia & 60.92 & 81.87 & 90.79 (3, 69) & 89.7 (2, 43) & 90.31 (5, 112)\\
%                          & Natives with the Internet & 69.21 & 90.45 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Bengali} & Gemini with 1 Wikipage (8 passage) & 43.78 & 52.97 & 60.61 (4, 265) & 55.12 (1, 271) & 58.03 (5, 536)\\
%                          & Gemini with 1 Wikipage (20 passage) & 52.56 & 63.53 & 69.11 (5, 206) & 65.68 (1, 207) & 67.49 (6, 413)\\
%                          & Gemini with Google Search (SAFE) & 75.55 & 87.95 & 86.82 (23, 67) & 87.79 (8, 66) & 87.28 (31, 133)\\
%                          & Gemini with knowledge generated by GPT-4 & 59.44 & 69.97 & 74.82 (9, 163) & 71.12 (4, 171) & 73.08 (13, 334)\\
%                          & Natives with Wikipedia & 57.83 & 61.22 & 74.08 (6, 154) & 62.71 (3, 163) & 68.74 (9, 317)\\
%                          & Natives with the Internet & 81.99 & 97.52 & 100 & 100 & 100\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{FActScore and agreement with golden labelling of introduced evaluation methods. Comparison is conducted on Gemini's generated facts (Gemini), GPT-4's generated facts (GPT-4) and a combine of both (Both). Gemini/Natives with Wiki (k) denotes using Gemini-Pro-1.0 for evaluation with k passages from 1 Wikipedia page as references. Gemini with Google API denotes using Gemini as the Internet search agent and evaluator (based on query results). Gemini with GPT-4's knowledge denotes using Gemini as the evaluator with GPT-4's generated knowledge and retrieved passages references. Natives with Wikipedia/Internet denotes natives, using 1 Wikipedia page or the entire Internet as references.}
% \label{tab:compare_proposed_method}
% \end{table*}

% (\#False positives, \#False negatives)

% namely increasing \# of passages, using GPT-4 to generate knowledge source and using Gemini as a Google search agent and evaluator, comparison with the baseline and native annotations


% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llccccc}
%     \toprule
%         \bf Lang & \bf Method & \multicolumn{2}{c}{\bf FActScore} & \multicolumn{3}{c}{\bf Agreement with golden labelling}\\
%         \cmidrule(r){3-4} \cmidrule(r){5-7}
%         & & \bf Gemini & \bf GPT-4 & \bf Gemini & \bf GPT-4 & \bf Both\\
%         \midrule
%         \mtr{7}{Spanish} & Gemini with Wiki (5) & 58.81 & 68.39 & 70.32 (36, 348) & 69.83 (9, 411) & 70.07 (45, 759)\\
%                          & Gemini with Wiki (8) & 63.29 & 72.84 & 74.34 (39, 293) & 73.99 (11, 351) & 74.16 (50, 644)\\
%                          & Gemini with Wiki (20) & 67 & 77.3 & 77.28 (44, 250) & 78.45 (11, 289) & 77.89 (50, 644)\\
%                          & Gemini with Google API & 81.45 & 90.3 & 83.23 (99, 118) & 89.87 (22, 119) & 86.67 (121, 237)\\
%                          & Gemini with GPT-4's knowledge & 78.83 & 93.46 & 84.62 (73, 126) & 91.88 (30, 83) & 88.38 (103, 209)\\
%                          & Natives with Wiki & 75.27 & 88.36 & 91.89 (3, 62) & 90.05 (1, 79) & 91.4 (4, 141) \\
%                          & Natives with Internet & 82.92 & 97.27 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Arabic} & Gemini with Wiki (8) & 56.4 & 73.71 & 77.91 (52, 212) & 78.33 (15, 187) & 78.09 (67, 399)\\
%                          & Gemini with Wiki (20) & 60.59 & 76.72 & 79.92 (65, 175) & 81.12 (16, 160) & 80.44 (81, 335)\\
%                          & Gemini with Google API & 72.3 & 87.66 & 80.25 (138, 101) & 86.27 (56, 82) & 82.89 (194, 183)\\
%                          & Gemini with GPT-4's knowledge & 64.44 & 82.4 & 83.6 (66, 130) & 84.66 (26, 117) & 84.06 (92, 247)\\
%                          & Natives with Wiki & 60.92 & 81.87 & 90.79 (3, 69) & 89.7 (2, 43) & 90.31 (5, 112)\\
%                          & Natives with Internet & 69.21 & 90.45 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Bengali} & Gemini with Wiki (8) & 43.78 & 52.97 & 60.61 (4, 265) & 55.12 (1, 271) & 58.03 (5, 536)\\
%                          & Gemini with Wiki (20) & 52.56 & 63.53 & 69.11 (5, 206) & 65.68 (1, 207) & 67.49 (6, 413)\\
%                          & Gemini with Google API & 75.55 & 87.95 & 86.82 (23, 67) & 87.79 (8, 66) & 87.28 (31, 133)\\
%                          & Gemini with GPT-4's knowledge & 59.44 & 69.97 & 74.82 (9, 163) & 71.12 (4, 171) & 73.08 (13, 334)\\
%                          & Natives with Wiki & 57.83 & 61.22 & 74.08 (6, 154) & 62.71 (3, 163) & 68.74 (9, 317)\\
%                          & Natives with Internet & 81.99 & 97.52 & 100 & 100 & 100\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{FActScore and agreement with golden labelling of introduced evaluation methods. Comparison is conducted on Gemini's generated facts (Gemini), GPT-4's generated facts (GPT-4) and a combine of both (Both). Gemini with Wiki (k) denotes using Gemini as the evaluator with k passages from 1 Wikipedia page as references. Gemini with Google API denotes using Gemini as the Internet search agent and evaluator (based on query results). Gemini with GPT-4's knowledge denotes using Gemini as the evaluator with GPT-4's generated knowledge and retrieved passages as references. Natives with Wiki/Internet denotes natives, using 1 Wikipedia page or the entire Internet as references for annotations.}
% \label{tab:compare_proposed_method}
% \end{table*}

% (\#False positives, \#False negatives)

% namely increasing \# of passages, using GPT-4 to generate knowledge source and using Gemini as a Google search agent and evaluator, comparison with the baseline and native annotations

\begin{table}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|cc|cc}
    \toprule
        & \mtr{2}{\bf Method} & \multicolumn{2}{c|}{\bf FActScore} & \multicolumn{2}{c}{\bf Accuracy}\\
        & & \bf GemP & \bf GPT4 & \bf GemP & \bf GPT4\\
        \midrule
        \mtr{6}{es} 
            % & GemP+Wiki (k=5) & 58.8 & 68.4 & 70.3 & 69.8\\
            & GemP+Wiki (k=8) & 63.3 & 72.8 & 74.3 & 74.0 \\
            & GemP+Wiki+T (k=8) & 63.3 & 72.8 & 74.3 & 74.0 \\
            & GemP+Wiki (k=20) & 67.0 & 77.3 & 77.3 & 78.5 \\
            & GemP+Google API & 81.5 & 90.3 & 83.2 & 89.9\\
            & GemP+GPT4's IK & 78.8 & 93.5 & 84.6 & 91.9\\
            \cline{2-6}
            & Natives+Wiki & 75.3 & 88.4 & 91.9 & 90.1\\
            & Natives+Internet & 82.9 & 97.3 & - & -\\
        \midrule
        \mtr{6}{ar} 
            & GemP+Wiki (k=8) & 56.4 & 73.7 & 77.9 & 78.3 \\
            & GemP+Wiki (k=20) & 60.6 & 76.7 & 79.9 & 81.1 \\
            & GemP+Google API & 72.3 & 87.7 & 80.3 & 86.3\\
            & GemP+GPT4's IK & 64.4 & 82.4 & 83.6 & 84.6 \\
            \cline{2-6}
            & Natives+Wiki & 60.9 & 81.9 & 90.8 & 89.7\\
            & Natives+Internet & 69.2 & 90.5 & - & -\\
        \midrule
        \mtr{6}{bn} 
            & GemP+Wiki (k=8) & 43.8 & 53.0 & 60.6 & 55.1 \\
            & GemP+Wiki (k=20) & 52.6 & 63.5 & 69.1 & 65.7\\
            & GemP+Google API & 75.6 & 88.0 & 86.8& 87.8\\
            & GemP+GPT4's IK & 59.4 & 70.0 & 74.8 & 71.1\\
            \cline{2-6}
            & Natives+Wiki & 57.8 & 61.2 & 74.1 & 62.7\\
            & Natives+Internet & 82.0 & 97.5 & - & - \\
        \bottomrule
    \end{tabular}
}
\caption{FActScore and agreement with golden labeling of introduced evaluation methods. Comparison is conducted on GemP and GPT4's generated facts (GPT4). GemP+Wiki (k=x) denotes using GemP as the evaluator with x passages from 1 Wikipedia page as references. GemP+Google API denotes using GemP as the Internet search agent and evaluator (evaluation is based on query results). GemP+GPT4's IK denotes using GemP as the evaluator with GPT-4's generated Internal Knowledge (IK) and retrieved passages as references. Natives+Wiki/Internet denotes natives, using 1 Wikipedia page or the entire Internet as references for annotations.}
\label{tab:compare_proposed_method}
\end{table}

==> tables/new_method_confusion.tex <==
\begin{table}[!h]
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|cccc|cccc}
    \toprule
        \mtr{2}{\bf Lang} 
        & \mtr{2}{\bf Method} 
        & \multicolumn{4}{c|}{\bf GemP} 
        & \multicolumn{4}{c}{\bf GPT4}\\
        & & \bf TP & \bf FN & \bf FP & \bf TN 
        & \bf TP & \bf FN & \bf FP & \bf TN\\
        \midrule
        \mtr{4}{es} 
            % & GemP+Wiki (k=5) & 58.8 & 68.4 & 70.3 & 69.8\\
            & GemP+Wiki (k=8)   & 60.3 & 22.6 & 3.0 & 14.1 & 72.1 & 25.2 & 0.8 & 1.9 \\
            & GemP+Wiki (k=20)  & 63.6 & 19.3 & 3.4 & 13.7 & 76.5 & 20.8 & 0.8 & 1.9\\
            & GemP+Google API   & 73.8 & 9.1 & 7.7 & 9.4 & 88.7 & 8.5 & 1.6 & 1.1\\
            & GemP+GPT4's IK    & 73.2 & 9.7 & 5.6 & 11.4 & 91.3 & 6.0 & 2.2 & 0.6 \\
        \midrule
        \mtr{4}{ar} 
            & GemP+Wiki (k=8)   & 52.1 & 17.7 & 4.4 & 25.9 & 72.1 & 20.1 & 1.6 & 6.2 \\
            & GemP+Wiki (k=20)  & 55.1 & 14.6 & 5.4 & 24.8 & 75.0 & 17.2 & 1.7 & 6.1 \\
            & GemP+Google API   & 60.8 & 8.5 & 11.5 & 19.2 & 81.7 & 8.8 & 6.0 & 3.5 \\
            & GemP+GPT4's IK    & 58.9 & 10.9 & 5.5 & 24.7 & 79.6 & 12.6 & 2.8 & 5.0 \\
        \midrule
        \mtr{4}{bn} 
            & GemP+Wiki (k=8)   & 43.2 & 38.8 & 0.6 & 17.4 & 52.8 & 44.7 & 0.2 & 2.3 \\
            & GemP+Wiki (k=20)  & 51.8 & 30.2 & 0.7 & 17.3 & 63.4 & 34.2 & 0.2 & 2.3 \\
            & GemP+Google API   & 72.2 & 9.8 & 3.4 & 14.6 & 86.6 & 10.9 & 1.3 & 1.2 \\
            & GemP+GPT4's IK    & 58.1 & 23.9 & 1.3 & 16.7 & 69.3 & 28.2 & 0.7 & 1.8 \\
        \bottomrule
    \end{tabular}
}
\caption{Source of errors the baseline model .}
\label{tab:compare_proposed_method_confusion}
\end{table}

% \begin{table}[!h]
% \centering
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{ll|cc|cc}
%     \toprule
%         \mtr{2}{\bf Lang} 
%         & \mtr{2}{\bf Method} 
%         & \multicolumn{2}{c|}{\bf GemP} 
%         & \multicolumn{2}{c}{\bf GPT4}\\
%         & &\bf FP & \bf FN & \bf FP & \bf FN \\
%         \midrule
%         \mtr{4}{es} 
%             % & GemP+Wiki (k=5) & 58.8 & 68.4 & 70.3 & 69.8\\
%             & GemP+Wiki (k=8)   & 39 & 293 &  11 & 351 \\
%             & GemP+Wiki (k=20)  & 44 & 250 &  11 & 289 \\
%             & GemP+Google API   & 99 & 118 &  22 & 119 \\
%             & GemP+GPT4's IK    & 73 & 126 &  30 & 83 \\
%         \midrule
%         \mtr{4}{ar} 
%             & GemP+Wiki (k=8)   & 52 & 212   &  15 & 187 \\
%             & GemP+Wiki (k=20)  & 65 & 175   &  16 & 160 \\
%             & GemP+Google API   & 138 & 101  &  56 & 82 \\
%             & GemP+GPT4's IK    & 66 & 130   &  26 & 117 \\
%         \midrule
%         \mtr{4}{bn} 
%             & GemP+Wiki (k=8)   & 4 & 265 & 1 & 271 \\
%             & GemP+Wiki (k=20)  & 5 & 206 & 1 & 207 \\
%             & GemP+Google API   & 23 & 67 & 8 & 66 \\
%             & GemP+GPT4's IK    & 9 & 163 & 4 & 171 \\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Source of errors the baseline model .}
% \label{tab:compare_proposed_method_confusion}
% \end{table}


% \begin{table*}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{llccccc}
%     \toprule
%         \bf Lang & \bf Method & \multicolumn{2}{c}{\bf FActScore} & \multicolumn{3}{c}{\bf Agreement with golden labelling}\\
%         \cmidrule(r){3-4} \cmidrule(r){5-7}
%         & & \bf Gemini & \bf GPT-4 & \bf Gemini & \bf GPT-4 & \bf Both\\
%         \midrule
%         \mtr{7}{Spanish} & Gemini with Wiki (5) & 58.81 & 68.39 & 70.32 (36, 348) & 69.83 (9, 411) & 70.07 (45, 759)\\
%                          & Gemini with Wiki (8) & 63.29 & 72.84 & 74.34 (39, 293) & 73.99 (11, 351) & 74.16 (50, 644)\\
%                          & Gemini with Wiki (20) & 67 & 77.3 & 77.28 (44, 250) & 78.45 (11, 289) & 77.89 (50, 644)\\
%                          & Gemini with Google API & 81.45 & 90.3 & 83.23 (99, 118) & 89.87 (22, 119) & 86.67 (121, 237)\\
%                          & Gemini with GPT-4's knowledge & 78.83 & 93.46 & 84.62 (73, 126) & 91.88 (30, 83) & 88.38 (103, 209)\\
%                          & Natives with Wiki & 75.27 & 88.36 & 91.89 (3, 62) & 90.05 (1, 79) & 91.4 (4, 141) \\
%                          & Natives with Internet & 82.92 & 97.27 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Arabic} & Gemini with Wiki (8) & 56.4 & 73.71 & 77.91 (52, 212) & 78.33 (15, 187) & 78.09 (67, 399)\\
%                          & Gemini with Wiki (20) & 60.59 & 76.72 & 79.92 (65, 175) & 81.12 (16, 160) & 80.44 (81, 335)\\
%                          & Gemini with Google API & 72.3 & 87.66 & 80.25 (138, 101) & 86.27 (56, 82) & 82.89 (194, 183)\\
%                          & Gemini with GPT-4's knowledge & 64.44 & 82.4 & 83.6 (66, 130) & 84.66 (26, 117) & 84.06 (92, 247)\\
%                          & Natives with Wiki & 60.92 & 81.87 & 90.79 (3, 69) & 89.7 (2, 43) & 90.31 (5, 112)\\
%                          & Natives with Internet & 69.21 & 90.45 & 100 & 100 & 100\\
%         \midrule
%         \mtr{6}{Bengali} & Gemini with Wiki (8) & 43.78 & 52.97 & 60.61 (4, 265) & 55.12 (1, 271) & 58.03 (5, 536)\\
%                          & Gemini with Wiki (20) & 52.56 & 63.53 & 69.11 (5, 206) & 65.68 (1, 207) & 67.49 (6, 413)\\
%                          & Gemini with Google API & 75.55 & 87.95 & 86.82 (23, 67) & 87.79 (8, 66) & 87.28 (31, 133)\\
%                          & Gemini with GPT-4's knowledge & 59.44 & 69.97 & 74.82 (9, 163) & 71.12 (4, 171) & 73.08 (13, 334)\\
%                          & Natives with Wiki & 57.83 & 61.22 & 74.08 (6, 154) & 62.71 (3, 163) & 68.74 (9, 317)\\
%                          & Natives with Internet & 81.99 & 97.52 & 100 & 100 & 100\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{FActScore and agreement with golden labelling of introduced evaluation methods. Comparison is conducted on Gemini's generated facts (Gemini), GPT-4's generated facts (GPT-4) and a combine of both (Both). Gemini with Wiki (k) denotes using Gemini as the evaluator with k passages from 1 Wikipedia page as references. Gemini with Google API denotes using Gemini as the Internet search agent and evaluator (based on query results). Gemini with GPT-4's knowledge denotes using Gemini as the evaluator with GPT-4's generated knowledge and retrieved passages as references. Natives with Wiki/Internet denotes natives, using 1 Wikipedia page or the entire Internet as references for annotations.}
% \label{tab:compare_proposed_method}
% \end{table*}

==> tables/retrieval_assessment.tex <==
% \begin{table}[!h]
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccc}
%     \toprule
%         \bf Lang & \bf Overlap out of 5 & \bf Top 1 included & \bf Top 2 included\\
%         \midrule
%         English & 67.7 & 85.8 & 94.61\\
%         \midrule
%         French  & 66.0 & 84.4 & 93.9\\
%         \midrule
%         Spanish & 66.13 & 84.8 & 94.26\\
%         \midrule
%         Russian  & 65.03 & 82.76 & 92.44\\
%         \midrule
%         Vietnamese  & 65.42 & 83.58 & 93.21\\
%         \midrule
%         Arabic  & 63.3 & 81.39 & 91.67\\
%         \midrule
%         Hindu  & 61.54 & 78.29 & 89.62\\
%         \midrule
%         Bengali  & 51.19 & 51.79 & 69.57\\
%         \bottomrule
%     \end{tabular}
% }
% \caption{Retrieval agreement between the multilingual retriever (cite here) and the original English retriever (cite here) through the number of overlapping passages retrieved by both retrievers out of retrieved 5 passages, included whether the most probable or at least one of the two most probable passages retrieved by the original English retriever is included in the 5 passages retrieved by the multilingual retriever}
% \label{tab:retrieval_assessment}
% \end{table}


\begin{table}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llccc}
    \toprule
        \bf Resource level & \bf Lang & \bf Overlap out of 5 & \bf Top 1 included & \bf Top 2 included\\
        \midrule
        \mtr{6}{High} & en & 67.70 & 85.80 & 94.61\\
        & fr  & 66.00 & 84.40 & 93.90\\
        & es & 66.13 & 84.80 & 94.26\\
        & ru  & 65.03 & 82.76 & 92.44\\
        & zh-cn  & 64.49 & 82.84 & 92.73\\
        & vi  & 65.42 & 83.58 & 93.21\\
        \midrule
        \mtr{2}{Medium} & ar  & 63.3 & 81.39 & 91.67\\
        & hi  & 61.54 & 78.29 & 89.62\\
        \midrule
        \mtr{1}{Low} & bn  & 51.19 & 51.79 & 69.57\\
        \bottomrule
    \end{tabular}
}
\caption{Retrieval agreement between the multilingual retriever (cite here) and the original English retriever (cite here) through the number of overlapping passages retrieved by both retrievers out of retrieved 5 passages, included whether the most probable or at least one of the two most probable passages retrieved by the original English retriever is included in the 5 passages retrieved by the multilingual retriever}
\label{tab:retrieval_assessment}
\end{table}

==> tables/retriever_vs_non_retriever_agreement_vs_gt.tex <==
\begin{table*}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|ccc|cccc|ccccc|cccc|cccc}
    \toprule
        \mtr{4}{\bf Lang} & \mtr{4}{\bf Subject }
        & \multicolumn{3}{c|}{\bf Natives} 
        & \multicolumn{4}{c|}{\bf GPT-4} 
        & \multicolumn{5}{c|}{\bf Gemini-Pro} 
        & \multicolumn{4}{c|}{\bf GPT-3.5-Turbo} 
        & \multicolumn{4}{c}{\bf Mistral}\\
        \cmidrule(r){3-5} 
        \cmidrule(r){6-9} 
        \cmidrule(r){10-14} 
        \cmidrule(r){15-18} 
        \cmidrule(r){19-22}
        % & & \bf Internet & \bf 1 Wikipage & \bf Entire Wikipedia & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/ retrieval (k=20) & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts\\
        % \midrule
        & & \bf Internet 
        & \bf Wikipedia
        & \bf Wikipedia
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        % \\
        & & &&
        & \bf (1 page)
        & \bf (All)
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        \\
        & & & & 
        & &
        & \bf (Translated)
        & \bf (Translated)
        & & \bf(k=20)
        & & \bf (Translated)
        & \bf (Translated)
        & & 
        & \bf (Translated)
        & \bf (Translated)
        & & 
        & \bf (Translated)
        & \bf (Translated)
        \\
        
        \midrule
        \mtr{2}{es} & Gemini & 100 & 92.1 & 95.0 & 86.2 & 86.0 & 84.9 & 85.0 & 70.1 & 77.18 & 76.2 & 69.0 & 73.1 & 81.3 & 79.3 & 81.7 & 78.0 & 77.9 & 61.2 & 78.2 & 69.3\\
                         & GPT-4 & 100 & 91.1 & 94.2 & 91.0 & 94.7 & 93.7 & 93.3 & 69.9 & 78.47 & 82.7 & 73.9 & 78.7 & 89.8 & 89.8 & 91.8 & 90.4 & 84.0 & 69.9 & 86.2 & 76.9\\
                         % & Both & 100 & 91.7 & 94.6 & 88.6 & 90.5 & 89.4 & 89.3 & 69.7 & 77.66 & 79.4 & 71.3 & 75.8 & 85.6 & 84.6 & 86.8 & 84.3 & 80.9 & 65.7 & 82.2 & 73.2\\
        \midrule
        \mtr{2}{ar} & Gemini & 100 & 91.1 & 93.7 & 85.9 & 75.3 & 84.1 & 79.0 & 78.2 & 80.16 & 68.5 & 76.3 & 68.7 & 79.5 & 67.6 & 82.6 & 77.1 & 73.4 & 54.5 & 81.6 & 68.6\\
                         & GPT-4 & 100 & 89.3 & 94.3 & 93.3 & 91.5 & 92.0 & 89.9 & 78.6 & 81.36 & 82.1 & 74.9 & 80.3 & 88.9 & 87.0 & 91.9 & 88.0 & 80.6 & 61.1 & 88.2 & 80.0\\
                         % & Both & 100 & 90.4 & 93.9 & 89.2 & 82.5 & 87.6 & 83.8 & 78.3 & 80.68 & 74.6 & 75.6 & 73.8 & 83.7 & 76.3 & 86.7 & 82.0 & 76.7 & 57.5 & 84.5 & 73.7\\
        \midrule
        \mtr{2}{bn} & Gemini & 100 & 73.9 & 76.4 & 86.0 & 79.9 & 84.0 & 82.8 & 60.3 & 68.95 & 72.7 & 67.0 & 72.5 & 65.2 & 71.5 & 79.6 & 80.2 & 55.6 & 57.2 & 73.3 & 68.7\\
                         & GPT-4 & 100 & 61.7 & 72.5 & 90.9 & 91.6 & 86.4 & 83.1 & 54.9 & 65.51 & 84.1 & 63.4 & 73.1 & 70.0 & 78.8 & 83.1 & 83.9 & 59.0 & 71.6 & 76.3 & 68.2\\
                         % & Both & 100 & 67.48 & 74.55 & 88.27 & 85.35 & 85.04 & 82.83 & 57.64 & 67.24 & 77.95 & 65.28 & 72.68 & 67.32 & 74.8 & 81.18 & 81.89 & 57.09 & 63.86 & 74.65 & 68.35\\
        \bottomrule
    \end{tabular}
}
\caption{Agreement of annotations by natives using different sources and modelling evaluators w/ different retrieval settings against golden labeling (natives navigating throughout the Internet to do evaluation.}
\label{tab:retriever_vs_without_retriever_agreement_gt}
\end{table*}


==> tables/retriever_vs_non_retriever_confusion_matrix.tex <==
\begin{table*}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{llcccccccccccccccccccc}
    \toprule
        \bf Lang & \bf Subject model & \multicolumn{2}{c}{\bf Natives} & \multicolumn{4}{c}{\bf GPT-4} & \multicolumn{5}{c}{\bf Gemini-Pro} & \multicolumn{4}{c}{\bf GPT-3.5-Turbo} & \multicolumn{4}{c}{\bf Mistral}\\
        \cmidrule(r){3-4} \cmidrule(r){4-7} \cmidrule(r){8-13} \cmidrule(r){14-17} \cmidrule(r){18-21}
        & & \bf access to 1 Wikipage & \bf access to the entire Wikipedia & \bf With retrieval & \bf Without retrieval & \bf With retrieval on translated facts & \bf Without retrieval on translated facts & \bf With retrieval & \bf With retrieval (20 retrieved passages) & \bf Without retrieval & \bf With retrieval on translated facts & \bf Without retrieval on translated facts & \bf With retrieval & \bf Without retrieval & \bf With retrieval on translated facts & \bf Without retrieval on translated facts & \bf With retrieval & \bf Without retrieval & \bf With retrieval on translated facts & \bf Without retrieval on translated facts\\
        \midrule
        \mtr{3}{Spanish} & Gemini & {'TT': 955, 'TF': 98, 'FT': 3, 'FF': 206} & {'TT': 993, 'TF': 60, 'FT': 3, 'FF': 206} & {'TT': 933, 'TF': 120, 'FT': 54, 'FF': 155} & {'TT': 991, 'TF': 62, 'FT': 115, 'FF': 94} & {'TT': 925, 'TF': 129, 'FT': 62, 'FF': 147} & {'TT': 975, 'TF': 79, 'FT': 110, 'FF': 99} & {'TT': 711, 'TF': 342, 'FT': 36, 'FF': 173} & {'TT': 809, 'TF': 244, 'FT': 44, 'FF': 165} & {'TT': 877, 'TF': 176, 'FT': 125, 'FF': 84} & {'TT': 712, 'TF': 50, 'FT': 341, 'FF': 159} & {'TT': 834, 'TF': 220, 'FT': 120, 'FF': 89} & {'TT': 924, 'TF': 129, 'FT': 107, 'FF': 102} & {'TT': 928, 'TF': 125, 'FT': 136, 'FF': 73} & {'TT': 946, 'TF': 107, 'FT': 124, 'FF': 85} & {'TT': 923, 'TF': 131, 'FT': 147, 'FF': 62} & {'TT': 842, 'TF': 211, 'FT': 68, 'FF': 141} & {'TT': 651, 'TF': 402, 'FT': 88, 'FF': 121} & {'TT': 860, 'TF': 193, 'FT': 82, 'FF': 127} & {'TT': 761, 'TF': 293, 'FT': 95, 'FF': 114}\\
                         & GPT-4 & {'TT': 1229, 'TF': 122, 'FT': 0, 'FF': 38} & {'TT': 1272, 'TF': 79, 'FT': 1, 'FF': 37} & {'TT': 1250, 'TF': 101, 'FT': 24, 'FF': 14} & {'TT': 1313, 'TF': 38, 'FT': 36, 'FF': 2} & {'TT': 1287, 'TF': 64, 'FT': 24, 'FF': 14} & {'TT': 1291, 'TF': 60, 'FT': 33, 'FF': 5} & {'TT': 942, 'TF': 409, 'FT': 9, 'FF': 29} & {'TT': 1063, 'TF': 288, 'FT': 11, 'FF': 27} & {'TT': 1141, 'TF': 210, 'FT': 31, 'FF': 7} & {'TT': 1001, 'TF': 350, 'FT': 13, 'FF': 25} & {'TT': 1083, 'TF': 268, 'FT': 28, 'FF': 10} & {'TT': 1236, 'TF': 115, 'FT': 27, 'FF': 11} & {'TT': 1240, 'TF': 111, 'FT': 31, 'FF': 7} & {'TT': 1267, 'TF': 84, 'FT': 30, 'FF': 8} & {'TT': 1249, 'TF': 102, 'FT': 31, 'FF': 7} & {'TT': 1151, 'TF': 200, 'FT': 22, 'FF': 16} & {'TT': 959, 'TF': 392, 'FT': 27, 'FF': 11} & {'TT': 1183, 'TF': 168, 'FT': 24, 'FF': 14} & {'TT': 1055, 'TF': 296, 'FT': 25, 'FF': 13}\\
                         & Both & {'TT': 2142, 'TF': 225, 'FT': 3, 'FF': 244} & {'TT': 2228, 'TF': 139, 'FT': 4, 'FF': 243} & {'TT': 2147, 'TF': 220, 'FT': 78, 'FF': 169} & {'TT': 2269, 'TF': 98, 'FT': 151, 'FF': 96} & {'TT': 2177, 'TF': 191, 'FT': 86, 'FF': 161} & {'TT': 2230, 'TF': 138, 'FT': 143, 'FF': 104} & {'TT': 1620, 'TF': 747, 'FT': 45, 'FF': 202} & {'TT': 1838, 'TF': 529, 'FT': 55, 'FF': 192} & {'TT': 1984, 'TF': 383, 'FT': 156, 'FF': 91} & {'TT': 1680, 'TF': 687, 'FT': 63, 'FF': 184} & {'TT': 1884, 'TF': 484, 'FT': 148, 'FF': 99} & {'TT': 2124, 'TF': 243, 'FT': 134, 'FF': 113} & {'TT': 2131, 'TF': 236, 'FT': 167, 'FF': 80} & {'TT': 2177, 'TF': 190, 'FT': 154, 'FF': 93} & {'TT': 2135, 'TF': 233, 'FT': 178, 'FF': 69} & {'TT': 1957, 'TF': 410, 'FT': 90, 'FF': 157} & {'TT': 1584, 'TF': 783, 'FT': 115, 'FF': 132} & {'TT': 2009, 'TF': 358, 'FT': 106, 'FF': 141} & {'TT': 1787, 'TF': 581, 'FT': 120, 'FF': 127}\\
        \midrule
        \mtr{3}{Arabic} & Gemini & {'TT': 692, 'TF': 99, 'FT': 1, 'FF': 332} & {'TT': 722, 'TF': 69, 'FT': 2, 'FF': 331} & {'TT': 701, 'TF': 90, 'FT': 68, 'FF': 265} & {'TT': 747, 'TF': 44, 'FT': 234, 'FF': 99} & {'TT': 675, 'TF': 116, 'FT': 63, 'FF': 270} & {'TT': 723, 'TF': 68, 'FT': 168, 'FF': 165} & {'TT': 596, 'TF': 195, 'FT': 50, 'FF': 283} & {'TT': 596, 'TF': 195, 'FT': 50, 'FF': 283} & {'TT': 635, 'TF': 156, 'FT': 198, 'FF': 135} & {'TT': 562, 'TF': 229, 'FT': 38, 'FF': 295} & {'TT': 601, 'TF': 190, 'FT': 162, 'FF': 171} & {'TT': 669, 'TF': 122, 'FT': 109, 'FF': 224} & {'TT': 676, 'TF': 115, 'FT': 249, 'FF': 84} & {'TT': 715, 'TF': 76, 'FT': 120, 'FF': 213} & {'TT': 705, 'TF': 86, 'FT': 171, 'FF': 162} & {'TT': 569, 'TF': 222, 'FT': 77, 'FF': 256} & {'TT': 386, 'TF': 405, 'FT': 107, 'FF': 226} & {'TT': 635, 'TF': 156, 'FT': 51, 'FF': 282} & {'TT': 562, 'TF': 229, 'FT': 124, 'FF': 209}\\
                         & GPT-4 & {'TT': 757, 'TF': 99, 'FT': 0, 'FF': 72} & {'TT': 803, 'TF': 53, 'FT': 0, 'FF': 72} & {'TT': 831, 'TF': 25, 'FT': 37, 'FF': 35} & {'TT': 844, 'TF': 12, 'FT': 67, 'FF': 5} & {'TT': 816, 'TF': 40, 'FT': 34, 'FF': 38} & {'TT': 824, 'TF': 32, 'FT': 62, 'FF': 10} & {'TT': 672, 'TF': 184, 'FT': 15, 'FF': 57} & {'TT': 672, 'TF': 184, 'FT': 15, 'FF': 57} & {'TT': 755, 'TF': 101, 'FT': 65, 'FF': 7} & {'TT': 635, 'TF': 221, 'FT': 12, 'FF': 60} & {'TT': 729, 'TF': 127, 'FT': 56, 'FF': 16} & {'TT': 789, 'TF': 67, 'FT': 36, 'FF': 36} & {'TT': 802, 'TF': 54, 'FT': 67, 'FF': 5} & {'TT': 821, 'TF': 35, 'FT': 40, 'FF': 32} & {'TT': 806, 'TF': 50, 'FT': 61, 'FF': 11} & {'TT': 702, 'TF': 154, 'FT': 26, 'FF': 46} & {'TT': 550, 'TF': 306, 'FT': 55, 'FF': 17} & {'TT': 771, 'TF': 85, 'FT': 25, 'FF': 47} & {'TT': 718, 'TF': 138, 'FT': 48, 'FF': 24}\\
                         & Both & {'TT': 1440, 'TF': 194, 'FT': 1, 'FF': 404} & {'TT': 1512, 'TF': 122, 'FT': 2, 'FF': 403} & {'TT': 1519, 'TF': 115, 'FT': 105, 'FF': 300} & {'TT': 1578, 'TF': 56, 'FT': 301, 'FF': 104} & {'TT': 1478, 'TF': 156, 'FT': 97, 'FF': 308} & {'TT': 1534, 'TF': 100, 'FT': 230, 'FF': 175} & {'TT': 1257, 'TF': 377, 'FT': 65, 'FF': 340} & {'TT': 1257, 'TF': 377, 'FT': 65, 'FF': 340} & {'TT': 1379, 'TF': 255, 'FT': 263, 'FF': 142} & {'TT': 1187, 'TF': 447, 'FT': 50, 'FF': 355} & {'TT': 1318, 'TF': 316, 'FT': 218, 'FF': 187} & {'TT': 1446, 'TF': 188, 'FT': 145, 'FF': 260} & {'TT': 1466, 'TF': 168, 'FT': 316, 'FF': 89} & {'TT': 1523, 'TF': 111, 'FT': 160, 'FF': 245} & {'TT': 1498, 'TF': 136, 'FT': 232, 'FF': 173} & {'TT': 1261, 'TF': 373, 'FT': 103, 'FF': 302} & {'TT': 929, 'TF': 705, 'FT': 162, 'FF': 243} & {'TT': 1394, 'TF': 240, 'FT': 76, 'FF': 329} & {'TT': 1269, 'TF': 365, 'FT': 172, 'FF': 233}\\
        \midrule
        \mtr{3}{Bengali} & Gemini & {'TT': 384, 'TF': 168, 'FT': 6, 'FF': 115} & {'TT': 399, 'TF': 153, 'FT': 6, 'FF': 115} & {'TT': 478, 'TF': 74, 'FT': 20, 'FF': 101} & {'TT': 496, 'TF': 56, 'FT': 79, 'FF': 42} & {'TT': 469, 'TF': 83, 'FT': 25, 'FF': 96} & {'TT': 491, 'TF': 61, 'FT': 55, 'FF': 66} & {'TT': 289, 'TF': 263, 'FT': 4, 'FF': 117} & {'TT': 348, 'TF': 204, 'FT': 5, 'FF': 116} & {'TT': 444, 'TF': 108, 'FT': 76, 'FF': 45} & {'TT': 333, 'TF': 219, 'FT': 3, 'FF': 118} & {'TT': 424, 'TF': 128, 'FT': 57, 'FF': 64} & {'TT': 358, 'TF': 194, 'FT': 40, 'FF': 81} & {'TT': 431, 'TF': 121, 'FT': 71, 'FF': 50} & {'TT': 453, 'TF': 99, 'FT': 38, 'FF': 83} & {'TT': 488, 'TF': 64, 'FT': 69, 'FF': 52} & {'TT': 278, 'TF': 274, 'FT': 25, 'FF': 96} & {'TT': 337, 'TF': 215, 'FT': 73, 'FF': 48} & {'TT': 392, 'TF': 160, 'FT': 20, 'FF': 101} & {'TT': 390, 'TF': 162, 'FT': 49, 'FF': 72}\\
                         & GPT-4 & {'TT': 369, 'TF': 219, 'FT': 3, 'FF': 12} & {'TT': 425, 'TF': 163, 'FT': 3, 'FF': 12} & {'TT': 543, 'TF': 45, 'FT': 10, 'FF': 5} & {'TT': 551, 'TF': 37, 'FT': 14, 'FF': 1} & {'TT': 513, 'TF': 75, 'FT': 7, 'FF': 8} & {'TT': 493, 'TF': 95, 'FT': 7, 'FF': 8} & {'TT': 317, 'TF': 271, 'FT': 1, 'FF': 14} & {'TT': 317, 'TF': 271, 'FT': 1, 'FF': 14} & {'TT': 506, 'TF': 82, 'FT': 14, 'FF': 1} & {'TT': 370, 'TF': 218, 'FT': 3, 'FF': 12} & {'TT': 435, 'TF': 153, 'FT': 9, 'FF': 6} & {'TT': 418, 'TF': 170, 'FT': 11, 'FF': 4} & {'TT': 474, 'TF': 114, 'FT': 14, 'FF': 1} & {'TT': 494, 'TF': 94, 'FT': 8, 'FF': 7} & {'TT': 501, 'TF': 87, 'FT': 10, 'FF': 5} & {'TT': 350, 'TF': 238, 'FT': 9, 'FF': 6} & {'TT': 426, 'TF': 162, 'FT': 9, 'FF': 6} & {'TT': 447, 'TF': 141, 'FT': 2, 'FF': 13} & {'TT': 402, 'TF': 186, 'FT': 6, 'FF': 9}\\
                         & Both & {'TT': 744, 'TF': 390, 'FT': 9, 'FF': 127} & {'TT': 818, 'TF': 316, 'FT': 9, 'FF': 127} & {'TT': 1015, 'TF': 119, 'FT': 30, 'FF': 106} & {'TT': 1041, 'TF': 93, 'FT': 93, 'FF': 43} & {'TT': 976, 'TF': 158, 'FT': 32, 'FF': 104} & {'TT': 978, 'TF': 156, 'FT': 62, 'FF': 74} & {'TT': 601, 'TF': 533, 'FT': 5, 'FF': 131} & {'TT': 660, 'TF': 474, 'FT': 6, 'FF': 130} & {'TT': 944, 'TF': 190, 'FT': 90, 'FF': 46} & {'TT': 699, 'TF': 435, 'FT': 6, 'FF': 130} & {'TT': 853, 'TF': 281, 'FT': 66, 'FF': 70} & {'TT': 770, 'TF': 364, 'FT': 51, 'FF': 85} & {'TT': 899, 'TF': 235, 'FT': 85, 'FF': 51} & {'TT': 941, 'TF': 193, 'FT': 46, 'FF': 90} & {'TT': 983, 'TF': 151, 'FT': 79, 'FF': 57} & {'TT': 623, 'TF': 511, 'FT': 34, 'FF': 102} & {'TT': 757, 'TF': 377, 'FT': 82, 'FF': 54} & {'TT': 834, 'TF': 300, 'FT': 22, 'FF': 114} & {'TT': 787, 'TF': 347, 'FT': 55, 'FF': 81}\\
        \bottomrule
    \end{tabular}
}
\caption{Confusion matrix of of annotations by natives using different sources and modelling evaluators with different retrieval settings against golden labeling (natives navigating throughout the Internet to do evaluation.}
\label{tab:retriever_vs_without_retriever_confusion_matrix}
\end{table*}


==> tables/retriever_vs_non_retriever_factscore.tex <==
\begin{table*}[!h]
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|ccc|cccc|ccccc|cccc|cccc}
    \toprule
        \mtr{4}{\bf Lang} & \mtr{4}{\bf Subject }
        & \multicolumn{3}{c|}{\bf Natives} 
        & \multicolumn{4}{c|}{\bf GPT-4} 
        & \multicolumn{5}{c|}{\bf Gemini-Pro} 
        & \multicolumn{4}{c|}{\bf GPT-3.5-Turbo} 
        & \multicolumn{4}{c}{\bf Mistral}\\
        \cmidrule(r){3-5} 
        \cmidrule(r){6-9} 
        \cmidrule(r){10-14} 
        \cmidrule(r){15-18} 
        \cmidrule(r){19-22}
        \cmidrule(r){3-5} \cmidrule(r){6-9} \cmidrule(r){10-14} \cmidrule(r){15-18} \cmidrule(r){19-22}
        % & & \bf Internet & \bf 1 Wiki page & \bf Entire Wikipedia & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/ retrieval (k=20) & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts & \bf w/ retrieval & \bf w/o retrieval & \bf w/ retrieval on translated facts & \bf w/o retrieval on translated facts\\
        % \midrule
        & & \bf Internet 
        & \bf Wikipedia
        & \bf Wikipedia
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        & \bf w/
        & \bf w/o
        % \\
        & & &
        & \bf (1 page)
        & \bf (All)
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        & \bf Retrieval
        % & \bf Retrieval
        \\
        & & & & 
        & &
        & \bf (Translated)
        & \bf (Translated)
        & & \bf(k=20)
        & & \bf (Translated)
        & \bf (Translated)
        & & 
        & \bf (Translated)
        & \bf (Translated)
        & & 
        & \bf (Translated)
        & \bf (Translated)
        \\
        \midrule
        \mtr{2}{es} & Gemini 
        & 82.7 & 75.4 & 78.3 & 78.2 & 87.6 & 78.2 & 95.9 & 59.2 & 67.6 & 79.4 & 60.4 & 75.6 & 81.7 & 84.3 & 84.8 & 84.7 & 72.1 & 58.6 & 74.6 & 67.8\\
        & GPT-4 & 97.3 & 88.4 & 91.7 & 91.7 & 97.1 & 94.4 & 95.3 & 68.4 & 77.3 & 84.4 & 73.0 & 80.0 & 90.9 & 91.5 & 93.4 & 92.2 & 84.4 & 71.0 & 86.9 & 77.7\\
        \midrule
        \mtr{2}{ar} & Gemini 
        & 70.4 & 61.6 & 64.4 & 68.4 & 87.3 & 65.7 & 79.3 & 57.5 & 57.5 & 74.1 & 53.4 & 67.9 & 69.2 & 82.3 & 74.3 & 77.9 & 57.5 & 43.9 & 61.0 & 61.0\\
        & GPT-4 & 92.2 & 81.5 & 86.5 & 93.5 & 98.2 & 91.6 & 95.5 & 74.0 & 74.0 & 88.4 & 69.7 & 84.6 & 88.9 & 93.6 & 92.8 & 93.4 & 78.5 & 65.2 & 85.8 & 82.5\\
        \midrule
        \mtr{2}{bn} & Gemini 
        & 81.8 & 57.5 & 60.1 & 74.0 & 85.4 & 73.4 & 81.1 & 43.5 & 52.5 & 77.3 & 49.9 & 71.5 & 59.1 & 74.6 & 73.0 & 82.8 & 45.0 & 60.9 & 61.2 & 65.2\\
        & GPT-4 & 97.5 & 60.2 & 60.6 & 91.7 & 93.7 & 86.3 & 82.9 & 52.7 & 52.7 & 86.2 & 61.9 & 73.6 & 71.1 & 80.9 & 83.3 & 84.7 & 59.5 & 72.1 & 74.5 & 67.7\\
        \bottomrule
    \end{tabular}
}
\caption{FActScore by natives using different sources and modeling evaluators w/ different retrieval settings.}
\label{tab:retriever_vs_w/o_retriever_factscore}
\end{table*}


